Drago: Primal-Dual Coupled Variance Reduction for Faster Distributionally Robust Optimization

We consider the penalized distributionally robust optimization (DRO) problem with a closed, convex uncertainty set, a setting that encompasses learning using $f$-DRO and spectral/$L$-risk minimization. We present Drago, a stochastic primal-dual algorithm that combines cyclic and randomized components with a carefully regularized primal update to achieve dual variance reduction. Owing to its design, Drago enjoys a state-of-the-art linear convergence rate on strongly convex-strongly concave DRO problems with a fine-grained dependency on primal and dual condition numbers. Theoretical results are supported by numerical benchmarks on regression and classification tasks.

==> _packages.tex <==
\usepackage{url}            %
\usepackage{booktabs}       %
\usepackage{amsfonts}       %
\usepackage{wrapfig}
\usepackage[mathscr]{euscript}
\usepackage{float}
\usepackage[nodisplayskipstretch]{setspace}
\usepackage[normalem]{ulem}


\RequirePackage{algorithm}
\RequirePackage{algorithmic}

\usepackage{times}
\usepackage{adjustbox}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{graphicx}
\usepackage{latexsym}
\usepackage{mathtools}
\usepackage{multirow}
\usepackage{paralist}
\usepackage{minitoc} %
\renewcommand \thepart{} %
\renewcommand \partname{} %
\usepackage{xspace}
\usepackage{enumitem}
\usepackage{thm-restate}
\usepackage{soul}

\usepackage{rotating}

\usepackage{tikz}
\usetikzlibrary{shapes}
\usetikzlibrary{positioning}
\usetikzlibrary{plotmarks}
\usetikzlibrary{patterns}
\usetikzlibrary{intersections,shapes.arrows}
\usetikzlibrary{fit,calc}

\newcommand*{\tikzmk}[1]{\tikz[remember picture,overlay,] \node (#1) {};\ignorespaces}
\newcommand{\boxit}[1]{\tikz[remember picture,overlay]{\node[yshift=3pt,fill=#1,opacity=.25,fit={(A)($(B)+(.95\linewidth,.8\baselineskip)$)}] {};}\ignorespaces}

\definecolor{darkpink}{rgb}{0.91, 0.33, 0.5}

\definecolor{puorange}{rgb}{0.80,0.20,0}
\definecolor{bluegray}{rgb}{0.04,0,0.7}
\definecolor{greengray}{rgb}{0.05,0.50,0.15}
\definecolor{darkbrown}{rgb}{0.40,0.2,0.05}
\definecolor{darkcyan}{rgb}{0,0.4,1}
\definecolor{black}{rgb}{0,0,0}
\definecolor{grey}{rgb}{0.93,0.93,0.93}
\definecolor{royalazure}{rgb}{0.0, 0.22, 0.66}
\definecolor{blueviolet}{RGB}{138,43,226}

\newcommand{\tabemph}[1]{\cellcolor{grey!30}\textcolor{black!50!royalazure}{#1}}%

\usepackage[colorlinks,citecolor=blue,linkcolor=blue,urlcolor=blue,breaklinks]{hyperref}
\newcommand{\orange}[1]{\textcolor{puorange}{#1}}
\newcommand{\violet}[1]{\textcolor{blueviolet}{#1}}


\usepackage[capitalize,noabbrev]{cleveref}

\crefname{section}{Sec.}{Sections}
\crefname{appendix}{Appx.}{Appxs}
\crefname{theorem}{Thm.}{Thms.}
\crefname{lemma}{Lem.}{Lems.}
\crefname{lem}{Lem.}{Lems.}
\crefname{corollary}{Cor.}{Cors.}
\crefname{proposition}{Prop.}{Props.}
\crefname{prop}{Prop.}{Props.}
\crefname{assumption}{Asm.}{Asms.}
\crefname{asm}{Asm.}{Asms.}
\crefname{algorithm}{Alg.}{Algs.}
\Crefname{algorithm}{Algorithm}{Algorithms}
\crefname{figure}{Fig.}{Figs.}
\crefname{table}{Tab.}{Tabs.}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}



\usepackage{color}
\definecolor{lightblue}{RGB}{0,160,200}
\definecolor{gray}{rgb}{0.4,0.4,0.4}
\usepackage{listings}
\lstset{ %
	basicstyle=\footnotesize\ttfamily,        %
	breaklines=true,                 %
	captionpos=b,                    %
	commentstyle=\color{gray},    %
	escapeinside={(*@}{@*)},          %
	keywordstyle=\color{lightblue},       %
	escapechar={|},
	tabsize=4
}

\newenvironment{proofsketch}{%
  \renewcommand{\proofname}{Proof Sketch}\proof}{\endproof}

\newenvironment{disproof}{%
  \renewcommand{\proofname}{Disproof}\proof}{\endproof}

\newcommand{\RM}[1]{{\color{greengray} [{\bf RM }: #1]}}
\newcommand{\ZH}[1]{{\color{RedViolet} [{\bf ZH}: #1]}}
\newcommand{\jd}[1]{{\color{purple}{\textbf{JD:} #1}}} 
\newcommand{\outline}[1]{{\color{royalazure} {\bf Outline }: #1}}

\newcommand{\ronak}{{\color{greengray} [{\bf RM }]}}
\newcommand{\zaid}{{\color{RedViolet} [{\bf ZH}]}}
\newcommand{\jelena}{{\color{purple}[{{\bf ZH}}]}} 


\newcommand{\red}[1]{{\color{purple}#1}}
\newcommand{\green}[1]{{\color{greengray}#1}}
\newcommand{\blue}[1]{{\color{royalazure}#1}}
\newcommand{\yellow}[1]{{\color{orange}#1}}
\newcommand{\purple}[1]{{\color{violet}#1}}

\newcommand{\edit}[1]{#1}


\newcommand{\myparagraph}[1]{\vspace{-8pt}\paragraph{#1}\hspace{-0.8em}}  %
\newcommand{\myparagraphsmall}[1]{\par\noindent\textit{{#1}.}}
  

